Prior-Dependent Allocations for Bayesian Fixed-Budget Best-Arm Identification in Structured Bandits

We study the problem of Bayesian fixed-budget best-arm identification (BAI) in structured bandits. We propose an algorithm that uses fixed allocations based on the prior information and the structure of the environment. We provide theoretical bounds on its performance across diverse models, including the first prior-dependent upper bounds for linear and hierarchical BAI. Our key contribution is introducing new proof methods that result in tighter bounds for multi-armed BAI compared to existing methods. We extensively compare our approach to other fixed-budget BAI methods, demonstrating its consistent and robust performance in various settings. Our work improves our understanding of Bayesian fixed-budget BAI in structured bandits and highlights the effectiveness of our approach in practical scenarios.

==> analysis.tex <==
\section{GENERAL PROOF SCHEME}\label{sec:analysis} 
We outline the key technical insights to derive our Bayesian proofs. The idea is general and can be applied to all our settings. Specific proofs for these settings are in \cref{sec:app_missing_proofs}.

\paragraph{From Frequentist to Bayesian proof.}To analyze their algorithm in the MAB setting, \citet{atsidakou2022bayesian} rely on the strong restriction that $\sigma_{0,i}=\sigma_0$ for all arms $i\in [K]$ and tune their allocations as a function of the noise variance $\sigma^2$ such that
in the Gaussian setting, the posterior variances $\hat{\sigma}_{n, i}^2$ in \eqref{eq:bayes_elim_posterior} are equal for all arms $i \in [K]$. This assumption is needed to directly leverage results from \citet{karnin2013almost}, thus allowing them to bound the frequentist PoE $\mathbb{P}\big(J_n \neq i_*(\theta) \mid \theta \big) \leq B(\theta)$ for a fixed instance $\theta$. 
Then, the expected PoE, $ \mathcal{P}_n = \E{}{\mathbb{P}\big(J_n \neq i_*(\theta) \mid \theta \big)}$, is bounded by computing $\E{\theta\sim P_0}{B(\theta)}$. We believe it is not possible to extend such technique for general choices of allocations $n_i$ and prior variances $\sigma^2_{0, i}$. Thus, we pursue an alternative approach, establishing the result in a fully Bayesian fashion. We start with a key observation.

\paragraph{Key reformulation of the expected PoE.} We observe that the expected PoE can be reformulated as follows
\begin{align*}%\label{eq:prob_misidenfication_rewritten}
\mathcal{P}_n &=  \E{}{\mathbb{P}\big(J_n \neq i_*(\theta) \mid \theta \big)}
%&= \mathbb{P}\big(J_n \neq i_*(\theta)\big)\nonumber\\
=  \E{}{\mathbb{P}\big(J_n \neq i_*(\theta) \mid H_n \big)}.
\end{align*}
This swap of measures means that to bound $\mathcal{P}_n$, we no longer bound the probability of
$$J_n = \argmax_{i \in [K]}\E{}{r(i; \theta) \,|\, H_n} \neq   \argmax_{i \in [K]} r(i; \theta) = i_*(\theta)$$
\emph{for any fixed $\theta$}. Instead, we only need to bound that probability \emph{when $\theta$ is drawn from the posterior distribution}. Precisely, we bound the probability that the arm $i$ maximizing the posterior mean $\E{}{r(i; \theta) \mid H_n}$ differs from the arm $i$ maximizing the posterior sample $r(i;\theta) \mid H_n$. This is achieved by first noticing that $\mathcal{P}_n$ can be rewritten as 
\begin{talign*}
\mathcal{P}_n = \sum_{\substack{i,j \in [K] \\ i \neq j}} \E{}{\mathbb{P}\left(i_*(\theta) = i \mid  J_n = j, H_n\right)\I{J_n = j}}.
\end{talign*}
The rest of the proof consists of bounding the above conditional probabilities for distincts $i$ and $j$, and this depends on the setting (MAB, linear or hierarchical). Roughly speaking, this is achieved as follows. $\mathbb{P}\left(i_*(\theta) = i \mid H_n, J_n = j\right)$ is the probability that arm $i$ maximizes the posterior sample $r(\cdot; \theta)$, given that arm $j$ maximizes the posterior mean $\E{}{r(\cdot; \theta) \mid H_n}$. We show that this probability decays exponentially with the squared difference $(\E{}{r(i; \theta)\,|\,H_n} - \E{}{r(j; \theta)\,|\,H_n})^2$. Taking the expectation of this term under the history $H_n$ gives the desired $\mathcal{O}(1/\sqrt{n})$ rate. All technical details and full explanations can be found in \cref{sec:app_missing_proofs}. This proof introduces a novel perspective for Bayesian BAI, distinguished by its tighter prior-dependent bounds on the expected PoE and ease of extension to more complex settings like linear and hierarchical bandits. However, its application to adaptive algorithms could be challenging, particularly due to the complexity of taking expectations under the history $H_n$ in that case. Also, extending this proof to non-Gaussian distributions is an interesting direction for future work. Note that \AdaBAI is applicable beyond the Gaussian case, as done in \cref{subsec:app_remarks_linear_models,subsec:experiments_GLB} featuring an approximate approach to logistic bandits \citep{chapelle11empirical}.







==> draft.tex <==
\begin{lemma}[Technical lemma]
\label{lemma:technical_lemma}
\todon{Replace all these bayesian calculus by a simple change of variable and just 1 technical lemma above}
    Let $A, C_x, C_{y}>0$ non negative constants, and $B \in \mathbb{R}$. Then
    $$
    \int_{\mathcal{X}}\int_{\mathcal{Y}}e^{-A(B + C_x x - C_y y)^2}\cN\left(x ; \mu_x, \sigma^2_x \right)\cN\left(y ;\mu_y, \sigma^2_y \right)dx dy = \frac{1}{\sqrt{1+2A C_x^2 \sigma^2_x + 2A C_y^2 \sigma^2_y}}e^{-\frac{A}{1+2A C_x^2 \sigma^2_x + 2A C_y^2 \sigma^2_y}\left(B + C_x \mu_x - C_y \mu_y\right)^2}\,.
    $$
\end{lemma}

\begin{proof}[Proof of \cref{lemma:technical_lemma}]
Let 
    \begin{align*}        
    I &= \int_{\mathcal{X}}\int_{\mathcal{Y}}e^{-A(B + C_x x - C_y y)^2}\cN\left(x ;\mu_x, \sigma^2_x \right)\cN\left(y ;\mu_y, \sigma^2_y \right)dx dy\\
    &=  e^{-AB^2}\int_{\mathcal{X}} e^{-AC_x^2x^2 - 2ABC_x x}I_y(x)\cN\left(x;\mu_x, \sigma^2_x\right)dx\,,
    \end{align*}
    where 
$$
I_y(x) = \int_{\mathcal{Y}}e^{-A\left(C_y y^2 - 2C_x C_y xy\right)+2ABC_y y }e^{-\frac{1}{2\sigma_y^2}(y - \mu_y)^2}\frac{1}{\sqrt{2\pi\sigma^2_y}}dy\,.
$$
Integrating with respect to variable $y$ gives 
\begin{align*}
    I_y(x)  = \frac{1}{\sqrt{\sigma_y^2 \Lambda_y}}e^{-\frac{1}{2\sigma_y^2}\mu_y^2 + Dx^2 + Fx + E}\,,
\end{align*}
where 
\begin{align*}
    \Lambda_y = 2AC_y^2 + \frac{1}{\sigma_y^2}\quad ; \quad D = \frac{2A^2 C_x^2 C_y^2 \sigma_y^2 }{2AC_y^2\sigma_y^2 + 1}\quad ; \quad E = \frac{\left(2ABC_y \sigma^2_y + \mu_y\right)^2}{2\sigma^2_y\left(2AC_y^2\sigma_y^2 + 1\right)}\quad ; \quad F = \frac{2AC_x C_y \left(2ABC_y\sigma_y^2 + \mu_y\right)}{2AC_y^2\sigma_y^2 + 1}\,.
\end{align*}
Therefore
\begin{align*}
I = \int_{\mathcal{X}} e^{-AC_x^2 x^2 - 2ABC_x x}e^{-\frac{1}{2\sigma_y^2}\mu_y^2 + Cdx^2 + Fx + E}e^{-\frac{1}{2\sigma_x^2}(x - \mu_x)^2}\frac{dx}{\sqrt{2\pi\sigma^2_x\sigma^2_y \Lambda_y}}\,.    
\end{align*}
Integrating with respect to variable $x$ gives
\begin{align*}
    I = \frac{1}{\sqrt{\sigma^2_x \Lambda_x \sigma^2_y \Lambda_y}}e^{-\frac{1}{2\sigma^2_y}\mu_y^2 -\frac{1}{2\sigma^2_x}\mu_x^2 + E + G}\,,
\end{align*}
where 
\begin{align*}
    \Lambda_x = 2AC_x^2 - 2D + \frac{1}{\sigma^2_x} \quad ; \quad G = \frac{\left(\mu_x + F\sigma^2_x - 2ABC_x \sigma^2_x\right)^2}{2\sigma_x^2\left(2AC_x^2\sigma_x^2 - 2D\sigma_x^2+1\right)}\,.
\end{align*}
After a few computations,
\begin{align*}
    I=\frac{1}{\sqrt{\sigma^2_x \Lambda_x \sigma^2_y \Lambda_y}}e^{(*)}\,,
\end{align*}
where 
\begin{align*}
    (*) &= -\frac{\mu_y^2}{2\sigma_y^2} - \frac{\mu_x^2}{2\sigma_x^2} + \frac{\mu_y^2}{2\sigma_y^2}\frac{1}{1 + 2AC_y^2\sigma_y^2} + \frac{2ABC_y}{1 + 2AC_y^2\sigma_y^2}\mu_y + \frac{2A^2B^2C_y^2\sigma_y^2}{1 + 2AC_y^2\sigma_y^2} + \frac{\mu_x^2}{2\sigma_x^2}\frac{2AC_y^2\sigma_y^2 + 1}{1 + 2AC_x^2 \sigma_x^2 + 2AC_y^2 \sigma_y^2} \\
    &+ \frac{2AC_x C_y}{1 + 2AC_x^2 \sigma_x^2 + 2AC_y^2 \sigma_y^2}\mu_x \mu_y - \frac{2AC_x B}{1 + 2AC_x^2 \sigma_x^2 + 2AC_y^2 \sigma_y^2}\mu_x + \frac{2A^2C_x^2(C_y \mu_y - B)^2 \sigma_x^2}{(2AC_y^2 + 1)(1 + 2AC_x^2 \sigma_x^2 + 2AC_y^2 \sigma_y^2)}\,.
\end{align*}
We recover the final results after a few more computations.    
\end{proof}


\subsection{On the tightness of our upper bound}
\label{subsec:app_experiments_tightness}
%\todon[inline]{On a simple problem, plot both performances of BayesElim and BAI-OPT, and plot the corresponding bound.}
We illustrate that our bound is non-vacuous for simple bandit instances. We consider the motivating setting of the introduction and of \cref{subsec:app_optimizing_allocations}, where $K=3$ and $\mu_0 = (2, 1.9, 0)$. In the first setting (hererogeneous setting), we set $\sigma_{0,1}=10^{-2}$ and $\sigma^2_{0, i}=0.5$ for $i \in \{2, 3\}$, while in the second setting (homogeneous setting), we set equal prior variances $\sigma_{0,i} = 0.5$ for any $i \in [3]$. We plot the expected PoE of \texttt{BAI-Uni}, \AdaBAIOpt and \BE and their corresponding upper bounds. Since the analysis of \texttt{BayesElim} \citep{atsidakou2022bayesian} is only valid in a homogeneous setting, we compute its upper bound for a prior mean variance $\sigma^2_0 = \frac{1}{K}\sum_{i \in [K]}\sigma^2_{0, i}$. The results are shown in \cref{fig:app_plotting_bound}, highlighting the tightness of our upper bound compared to the upper bound of \citet{atsidakou2022bayesian}. We do the same experiments for $K=5$ arms with prior mean $\mu_0 = (2, 1.9, 0, 0, 0)$, and prior variance $\sigma^2_{0, i}=0.5$ for $i \in \{3, 4, 5\}$. Results are shown in \cref{fig:app_plotting_bound_5_arms}. The significant discrepancy is due to the multiplicative constant in their bound, which our new proof techniques allowed us to remove. 

\todon{Maybe put in the main}
\begin{figure}[H]
\centering
\includegraphics[width=15cm]{figures/app_plotting_bounds.pdf}
\caption{Average PoE of \texttt{BAI-Uni}, \AdaBAIOpt and their corresponding upper bounds (UB) for two settings with $K=3$ arms.} 
\label{fig:app_plotting_bound}
\end{figure}

\begin{figure}[H]
\centering
\includegraphics[width=15cm]{figures/app_plotting_bounds_5_arms.pdf}
\caption{Average PoE of \texttt{BAI-Uni}, \AdaBAIOpt and their corresponding upper bounds (UB) for two settings with $K=5$ arms.} 
\label{fig:app_plotting_bound_5_arms}
\end{figure}



\textbf{Bayesian simple regret minimization.} \citet{komiyama2023rate} provides rate-optimal bound on the Bayesian simple regret. This bound scales as $\mathcal{O}(1/n)$ when considering Bernoulli reward distributions. We recall that considering Bayesian simple regret or expected PoE can lead to different rates \citep{komiyama2023rate}. Previous works also obtained this rate on the Bayesian simple regret, by using algorithms designed for regret minimization. More precisely, a policy having a regret upper bounded as $\mathcal{O}(1/n)$ implies an upper bound on the Bayesian simple regret of $\mathcal{O}(1/\sqrt{n})$ \citep{russo2018learning,azizi2023meta}. \citet{komiyama2022suboptimal} designed a Bayes-optimal policy (optimal with respect to the Bayesian simple regret). It is proven that this algorithm cannot have an exponential rate for the upper bound, and its Bayesian simple regret is polynomially small to $n$.

\textbf{Structured Bayesian bandits.} The idea of using G-optimal design for pure exploration in frequentist linear bandit is not new \citep{azizi2021fixed,yang2022minimax}. Recent papers approached the problem of learning in Bayesian bandits instances with two-level structure \citep{kveton21metathompson,basu21noregrets,hong22hierarchical,aouali2022mixed,peleg2022metalearning}. Our work is the first one that uses such Bayesian hierarchical structure for PoE minimization in BAI. \todon{Put more references concerning hierarchical bayesian models}

\textbf{Lower bounds for Fixed-budget BAI.} Existing lower bounds on PoE in fixed-budget BAI are only valid in the frequentist setting \citep{carpentier2016tight}. \citet{atsidakou2022bayesian} states the existence of a prior distribution for which the expected PoE over this distribution is lower bounded by $\mathcal{O}(1/\sqrt{n})$. This gives an intuition of why having an upper bound of $\mathcal{O}(1/\sqrt{n})$ on the expected PoE is coherent. However, this can not be seen as a general lower bound for the Bayesian BAI, since we want to lower bound the expected PoE of a class of policy given any prior distribution. \citet{komiyama2023rate} gives such result, stating a lower bound of $\mathcal{O}(1/n)$ for the Bayesian simple regret. In the frequentist setting, the simple regret is lower bounded by the PoE when the mean rewards are in $[0, 1]$. This relation does not hold in the Bayesian setting for Gaussian prior, but would hold for the Bernoulli reward case. In such case, a rate of $\mathcal{O}(1/\sqrt{n})$ would be consistent with this result.

\subsection{Beyond Gaussian distributions in standard model}
\label{subsec:app_remarks_linear_models}

The standard model is a general Bayesian model. We first recall its general form,
\begin{align*}
   \theta_i &\sim P_{0, i}  & \forall i \in [K]\nonumber\\
    Y_t \mid \theta, A_t &\sim P(\cdot; \theta_{A_t})  & \forall t \in [n]\,.
\end{align*}
\todon{Mention GLB here}
Our algorithms \AdaBAIFixed and \AdaBAI can be used for other distributions than Gaussian rewards with Gaussian prior. One requirement to get closed-form posterior means is to have a conjugate prior for the reward distribution. This is the case for any reward distribution belonging to an exponential family distribution. For example, in the Beta-Bernoulli conjugate setting, the priors for the $\theta_i$ are Beta distributions, while the conditional distribution of $Y_t$ conditioned on $\theta$ and $A_t$ follows a Bernoulli distribution with parameter $\theta_{A_t}$:
\begin{align}
\label{eq:standard_bernoulli}
   \theta_i &\sim \rm{Beta}(\alpha_{0, i}, \beta_{0, i}) & \forall i \in [K]\nonumber\\
    Y_t \mid \theta, A_t &\sim \mathcal{B}(\theta_i(A_t))  & \forall t \in [n]\,,
\end{align}
where $(\alpha_{0, i})_{i \in [K]}$ and $(\beta_{0, i})_{i \in [K]}$ are known hyperparameters. The posterior mean distribution given the history $H_n$ containing $n_i$ samples from arm $i$ is a Beta distribution $\rm{Beta}(\hat\alpha_{n, i}, \hat\beta_{n, i})$ with
\begin{align*}
    \hat\alpha_{n, i} = \alpha_{0, i} + \sum_{t \in \mathcal{T}_i} \I{Y_t = 1} ; \quad \hat\beta_{n, i} = \beta_{0, i} + \sum_{t \in \mathcal{T}_i} \I{Y_t = 0}\,,
\end{align*}
where we recall $\mathcal{T}_i = \{t \in[n], A_t = i\}$.
\todon{discuss GLB}













\begin{theorem}[Complete statement of \cref{th:upper_bound_hierarchical_model}]
\label{th:complete_upper_bound_hierarchical_model}
    The expected PoE of \emph{\AdaBAIFixed} under the hierarchical Gaussian model in \eqref{eq:model_gaussian} instantiated with arbitrary allocation weights $\omega \in \Delta_K^+$ is upper bounded as
    \begin{align*}
    \mathcal{P}_n \leq \sum_{i \in [K]}\sum_{j \in [K]\setminus \{i\}} \frac{\xi_j}{\sqrt{1 + \frac{\lambda_{i, j}}{\hat{\sigma}^2_{n, i} + \hat{\sigma}^2_{n, j}}}}e^{-\frac{\lVert b_i - b_j \rVert^2_{\nu \nu^\top}}{ 2(\hat{\sigma}^2_{n, i} + \hat{\sigma}^2_{n, j} + \lambda_{i, j}) }}\,,
    \end{align*}
where 
\begin{tiny} % can also use small instead, it's the appendix, it's okay
    \begin{align*}
    &\lambda_{i, j} = \mathbb{V}(\hat \mu_i + \hat\mu_j) = \frac{\sigma^4_{0, i}}{(\sigma^2_{0, i}\omega_i n + \sigma^2)^2}\mathbb{V}(B_i) + \frac{\sigma^4_{0, j}}{(\sigma^2_{0, j}\omega_j n + \sigma^2)^2}\mathbb{V}(B_j)\\
    &+\frac{\sigma^4}{(\sigma^2_{0, i}\omega_i n + \sigma^2)^2}\sum_{k \in [K]}\frac{(b_k^\top P^{-1}b_i)^2}{(\sigma^2 + \omega_k n\sigma^2_{0, k})^2}\mathbb{V}(B_k) +  \frac{\sigma^4}{(\sigma^2_{0, j}\omega_j n + \sigma^2)^2}\sum_{k \in [K]}\frac{(b_k^\top P^{-1}b_j)^2}{(\sigma^2 + \omega_kn\sigma^2_{0, k})^2}\mathbb{V}(B_k)\\
    &+ \frac{\sigma^4}{(\sigma^2_{0, i}\omega_i n + \sigma^2)^2}\sum_{k \in [K]}\sum_{k^\prime \in [K]\setminus\{k\}} \frac{(b_k^\top P^{-1}b_i).(b_{k^\prime}^\top P^{-1}b_i)}{(\sigma^2_{0, k}\omega_k n + \sigma^2).(\sigma^2_{0, k^\prime}\omega_{k^\prime} n + \sigma^2)}\cov(B_k, B_{k^\prime}) \\
    &+ \frac{\sigma^4}{(\sigma^2_{0, j}\omega_j n + \sigma^2)^2}\sum_{k \in [K]}\sum_{k^\prime \in [K]\setminus\{k\}} \frac{(b_k^\top P^{-1}b_j).(b_{k^\prime}^\top P^{-1}b_j)}{(\sigma^2_{0, k}\omega_k n + \sigma^2).(\sigma^2_{0, k^\prime}\omega_{k^\prime} n + \sigma^2)}\cov(B_k, B_{k^\prime})\\
    &+ \frac{2\sigma^4}{(\sigma^2_{0, i}\omega_i n + \sigma^2)(\sigma^2_{0, j}\omega_j n + \sigma^2)} \left[\sum_{k \in [K]}\frac{(b_k^\top P^{-1} b_i)(b_k^\top P^{-1}b_j)}{(\sigma^2 + \omega_k n \sigma^2_{0, k})^2}\mathbb{V}(B_k) + \sum_{k \in [K]}\sum_{k^\prime \in [K]\setminus\{k\}} \frac{(b_k^\top P^{-1}b_i).(b_{k^\prime}^\top P^{-1}b_j)}{(\sigma^2_{0, k}\omega_k n + \sigma^2).(\sigma^2_{0, k^\prime}\omega_{k^\prime} n + \sigma^2)}\cov(B_k, B_{k^\prime})\right]\\
    &+ \frac{2\sigma^2_{0, i}\sigma^2_{0, j}}{(\sigma^2_{0, i}\omega_i n + \sigma^2)(\sigma^2_{0, j}\omega_j n + \sigma^2)}\cov(B_i, B_j) \\
    &+ \frac{2\sigma^2\sigma^2_{0, i}}{(\sigma^2_{0, i}\omega_i n + \sigma^2)^2}\left[\sum_{k \in [K]\setminus \{i\}} \frac{b_k^\top P^{-1}b_i}{(\sigma^2_{0, k}\omega_k n + \sigma^2)}\cov(B_k, B_i) + \frac{b_i^\top P^{-1}b_i}{(\sigma^2_{0, i}\omega_i n + \sigma^2)}\mathbb{V}(B_i)\right]\\
    &+ \frac{2\sigma^2\sigma^2_{0, j}}{(\sigma^2_{0, j}\omega_j n + \sigma^2)^2}\left[\sum_{k \in [K]\setminus \{j\}} \frac{b_k^\top P^{-1}b_j}{(\sigma^2_{0, k}\omega_k n + \sigma^2)}\cov(B_k, B_j) + \frac{b_j^\top P^{-1}b_i}{(\sigma^2_{0, j}\omega_j n + \sigma^2)}\mathbb{V}(B_j)\right]\\
    &+ \frac{2\sigma^2 \sigma^2_{0, j}}{(\sigma^2_{0, i}\omega_i n + \sigma^2)(\sigma^2_{0, j}\omega_j n + \sigma^2)}\left[\sum_{k \in [K]\setminus\{j\}}\frac{b_k^\top P^{-1}b_i}{\sigma^2 + \omega_k n \sigma^2_{0, k}}\cov(B_k, B_i) + \frac{b_j^\top P^{-1}b_i}{\sigma^2 + \omega_jn\sigma^2_{0, j}}\mathbb{V}(B_j)\right]\\
    &+ \frac{2\sigma^2 \sigma^2_{0, i}}{(\sigma^2_{0, j}\omega_j n + \sigma^2)(\sigma^2_{0, i}\omega_i n + \sigma^2)}\left[\sum_{k \in [K]\setminus\{i\}}\frac{b_k^\top P^{-1}b_j}{\sigma^2 + \omega_k n \sigma^2_{0, k}}\cov(B_k, B_j) + \frac{b_i^\top P^{-1}b_j}{\sigma^2 + \omega_i n\sigma^2_{0, i}}\mathbb{V}(B_i)\right]\,,
\end{align*}
\end{tiny}
and
\begin{align*}
    P = \Sigma^{-1} + \sum_{k \in [K]}\frac{\omega_k n}{\sigma^2 + \omega_k n \sigma^2_{0, k}}b_k b_k^\top\quad ; \quad \mathbb{V}(B_k) =  \omega_k n \sigma^2 + \omega_k^2 n^2 (\sigma^2_{0, k} +b_k^\top \Sigma b_k) \quad ; \quad \cov(B_k, B_{k^\prime}) = \omega_k \omega_{k^\prime}n^2 b_k^\top \Sigma b_{k^\prime}\,.
\end{align*}

\end{theorem}

\begin{proof}[Proof of \cref{th:complete_upper_bound_hierarchical_model}]
This proof follows the same idea of the proof of \cref{th:upper bound}. We first write $\mathcal{P}_n$ as in \cref{eq:double_sum_probabilities},
\begin{align*}
    \mathcal{P}_n &= \sum_{i\in [K]}\sum_{j \in [K]}\I{i \neq j}\E{}{\mathbb{P}(i_*(\theta)=i \mid J_n = j, H_n)\I{J_n = j}}\\
    &= \sum_{i \in [K]}\sum_{j \in [K]\setminus\{i\}}\E{}{\mathbb{P}(i_*(\theta)=i \mid J_n = j, H_n)}\mathbb{P}(J_n = j)\,.
\end{align*}

\textbf{Upper bounding first term of the sum.}

Following \eqref{eq:Hoeffding_2},
\begin{align*}
    \mathbb{P}(i_*(\theta)=i \mid J_n = j, H_n)\leq e^{-\frac{(\hat\mu_j - \hat\mu_i)^2}{2(\hat\sigma^2_i + \hat\sigma^2_j)}}\,,
\end{align*}
where $\hat\mu_i$ and $\hat\sigma^2_i$ are given by \eqref{eq:posterior}. Taking the expectation with respect to the history $H_n$,
\begin{align*}
  \E{}{\mathbb{P}(i_*(\theta)=i \mid J_n = j, H_n)}\leq \E{}{e^{-\frac{(\hat\mu_j - \hat\mu_i)^2}{2(\hat\sigma^2_i + \hat\sigma^2_j)}}}\,.
\end{align*}
Since $\hat\mu_i - \hat\mu_j \sim \cN\big( \E{}{\hat\mu_i}-\E{}{\hat\mu_j}, \mathbb{V}(\hat\mu_i)+\mathbb{V}(\hat\mu_j) \big)$, applying \cref{lemma:integration_gaussian} gives
\begin{align*}
    \E{}{e^{-\frac{(\hat\mu_j - \hat\mu_i)^2}{2(\hat\sigma^2_i + \hat\sigma^2_j)}}} &= \frac{1}{\sqrt{1 + \frac{\mathbb{V}(\hat\mu_i + \hat\mu_j)}{\hat\sigma^2_i + \hat\sigma^2_j}}}e^{-\frac{(\E{}{\hat\mu_i} - \E{}{\hat\mu_j})^2}{2(\hat\sigma^2_i + \hat\sigma^2_j)}\frac{1}{1 + \frac{\mathbb{V}(\hat\mu_i + \hat\mu_j)}{\hat\sigma^2_i + \hat\sigma^2_j}}}
\end{align*}
So that :
\begin{align}\label{eq:temp eq 1 hierarchical model}
    \E{}{\mathbb{P}(i_*(\theta)=i \mid J_n = j, H_n)}\leq \frac{1}{\sqrt{1 + \frac{\mathbb{V}(\hat\mu_i + \hat\mu_j)}{\hat\sigma^2_i + \hat\sigma^2_j}}}e^{-\frac{\left(\E{}{\hat\mu_i} - \E{}{\hat\mu_j}\right)^2}{2\left(\hat\sigma^2_i + \hat\sigma^2_j + \mathbb{V}(\hat\mu_i + \hat\mu_j) \right)}}\,.
\end{align}

By the law of total variance;
\begin{align*}
    \mathbb{V}(\theta_i + \theta_j) &= \E{}{\mathbb{V}(\theta_i + \theta_j \mid H_n)} + \mathbb{V}(\E{}{\theta_i + \theta_j \mid H_n})\\
    &= \hat\sigma^2_{n, i}+ \hat\sigma^2_{n, j}+\mathbb{V}(\hat\mu_{n, i})+\mathbb{V}(\hat\mu_{n, j})\,,
\end{align*}
where $\mathbb{V}(\theta_i + \theta_j) = \sigma^2_{0, i} + \sigma^2_{0,j} + b_i^\top \Sigma b_i + b_j^\top \Sigma b_j$.

\textbf{Upper bounding second term of the sum.}

We introduce $m = \argmax{i \in [K]} \E{}{\hat\mu_i}$ and apply Hoeffding inequality as in \eqref{eq:Hoeffding_1},
\begin{align*}
    \mathbb{P}(J_n = j) &\leq \mathbb{P}(\hat\mu_j \geq \hat\mu_m) \leq e^{-\frac{\left(\E{}{\hat\mu_j}-\E{}{\hat\mu_m}\right)^2}{\mathbb{V}_{}(\hat\mu_j + \hat\mu_m)}}\,.
\end{align*}

\textbf{Computing Covariances term.}

The rest of the proof is to compute $\E{}{\hat\mu_i}$ and $\mathbb{V}(\hat\mu_i + \hat\mu_j)$ for any pair of arms $(i, j)$. Denoting $Q$ the latent prior $\mu \sim Q$,

\begin{align*}
    \pi_{H_n}(H_n) &= \pi_{H_n}(Y_{A_1}, ..., Y_{A_n})\\
    &= \iint_{(\theta, \mu)}\mathcal{L}_{\theta}(Y_{A_1}, ..., Y_{A_n})P_0(\theta\mid\mu)Q(\mu)d\theta d\mu\\
    &= \iint_{(\theta, \mu)} \prod_{i \in [K]}\mathcal{L}_{\theta_i}\left((Y_{t})_{t \in \mathcal{T}_i}\right)P_{0, i}(\theta_i\mid\mu)Q(\mu)d\theta_i d\mu\\
    &= \int_{\mu}\left[ \prod_{i\in [K]}\int_{\theta_i}\cN\left((Y_t)_{t \in \mathcal{T}_i}) ; \theta_i\bm{1}_{\omega_i n}, \sigma^2 I_{\omega_i n}\right)\cN(\theta_i ; b_i^\top \mu, \sigma^2_{0, i})d\theta_i \right]Q(\mu)d\mu\,.
\end{align*}
From properties of Gaussian convolutions \citep{Bishop2006},
\begin{align*}
    \int_{\theta_i}\cN\left((Y_{t})_{t \in \mathcal{T}_i}) ; \theta_i\bm{1}_{\omega_i n}, \sigma^2 I_{\omega_i n}\right)\cN(\theta_i ; b_i^\top \mu, \sigma^2_{0, i})d\theta_i  &= \cN\left((Y_{t})_{t \in \mathcal{T}_i}) ; (b_i^\top\mu)\bm{1}_{\omega_i n}, \sigma^2. I_{\omega_i n} + \bm{1}_{\omega_i n}\bm{1}_{\omega_i n}^\top \sigma^2_{0, i} \right)\,.
\end{align*}
Therefore,
\begin{align*}
    &\prod_{i \in [K]}\int_{\theta_i}\cN\left((Y_{t})_{t \in \mathcal{T}_i}) ; \theta_i\bm{1}_{\omega_i n}, \sigma^2 I_{\omega_i n}\right)\cN(\theta_i ; b_i^\top \mu, \sigma^2_{0, i})d\theta_i\\
    &= \cN(H_n ; \sum_{i \in [K]}e_i^{\mathbb{R}^K} \otimes\left(\sum_{t\in [\omega_i n]}\Tilde{e}_t^{\mathbb{R}^{\omega_i n}} \otimes b_i^\top\right)\otimes \mu, \, I_K \otimes (\sigma^2 I_{\omega_i n} + \bm{1}_{\omega_i n}\bm{1}_{\omega_i n}^\top \sigma^2_{0, i}))\,,
\end{align*}
where we define $e_i^{\mathbb{R}^K}$ as the $i^{th}$ base vector of $\mathbb{R}^K$ and $\Tilde{e}_i^{\mathbb{R}^{\omega_i n}}$ as the $t^{th}$ base vector of $\mathbb{R}^{\omega_i n}$.

Therefore,
\begin{align*}
    \pi(H_n) &= \int_{\mu}\cN(H_n ; \sum_{i \in [K]}e_i^{\mathbb{R}^K} \otimes\left(\sum_{t\in [\omega_i n]}\Tilde{e}_t^{\mathbb{R}^{\omega_i n}} \otimes b_i^\top\right)\otimes \mu, \, I_K \otimes (\sigma^2 I_{\omega_i n} + \bm{1}_{\omega_i n}\bm{1}_{\omega_i n}^\top \sigma^2_{0, i}))\cN(d\mu;\nu, \Sigma)\\
    &= \cN(H_n ; \check{\mu}, \check{\Sigma})\,,
\end{align*}
where $\check{\mu}\in \mathbb{R}^n$, $\check{\Sigma}\in \mathbb{R}^{n\times n}$ with
\begin{align}\label{eq:marginal posterior hierarchical}
    &\check{\mu} = \sum_{i \in [K]}e_i^{\mathbb{R}^K} \otimes\left(\sum_{t\in [\omega_i n]}\Tilde{e}_t^{\mathbb{R}^{\omega_i n}} \otimes b_i^\top\right)\otimes \nu\\
    &\check{\Sigma} = I_K \otimes (\sigma^2 I_{\omega_i n} + \bm{1}_{\omega_i n}\bm{1}_{\omega_i n}^\top \sigma^2_{0, i}) + \left[\sum_{i \in [K]}e_i^{\mathbb{R}^K} \otimes\left(\sum_{t\in [\omega_i n]}\Tilde{e}_t^{\mathbb{R}^{\omega_i n}} \otimes b_i^\top\right)\right] \Sigma \left[\sum_{i \in [K]}e_i^{\mathbb{R}^K} \otimes\left(\sum_{t\in [\omega_i n]}\Tilde{e}_t^{\mathbb{R}^{\omega_i n}} \otimes b_i^\top\right)\right]^\top \,.
\end{align}
%\todon[inline]{Maybe give a comprenhensive description of the covariance matrix}
The covariance matrix $\check{\Sigma}$ seems complex but has a simple structure. The first term $I_K \otimes (\sigma^2 I_{\omega_i n} + \bm{1}_{\omega_i n}\bm{1}_{\omega_i n}^\top \sigma^2_{0, i})$ is the same as in the standard model. The remaining term accounts for the correlation between distinct arms $(i, j)$, and this correlation is of the form $b_i^\top \Sigma b_j$.

Now we are ready to compute $\E{}{\hat\mu_i}$ fot any arm $k\in[K]$: from \eqref{eq:model_gaussian},
\begin{align*}
    \E{}{\hat\mu_k} &=\E{}{ \frac{\sigma^2\sigma^2_{0, i}}{\sigma^2_{0, k}\omega_k n + \sigma^2}\left(\frac{\hat\mu^\top b_k}{\sigma^2_{0, k}}+\frac{B_k}{\sigma^2}\right)}= \frac{\sigma^2}{\sigma^2_{0, k}\omega_k n + \sigma^2}\E{}{\hat\mu^\top b_k} + \frac{\sigma^2_{0, k}}{\sigma^2_{0, k}\omega_k n + \sigma^2}\E{}{B_k}\,.
\end{align*}
Then,
\begin{align*}
    \hat\mu^\top b_k &= \left( \nu^\top \Sigma^{-1} + \sum_{i \in [K]}\frac{B_i}{\sigma^2 + \omega_i n \sigma^2_{0, i}}b_i^\top \right)\left(\Sigma^{-1} + \sum_{i \in [K]}\frac{\omega_i n}{\sigma^2 + \omega_i n \sigma^2_{0, i}}b_i b_i^\top\right)^{-1}b_k\\
    &= \nu^\top \Sigma^{-1}\left(\Sigma^{-1} + \sum_{i \in [K]}\frac{\omega_i n}{\sigma^2 + \omega_i n \sigma^2_{0, i}}b_i b_i^\top\right)^{-1}b_k + \sum_{i \in [K]}\frac{B_i}{\sigma^2 + \omega_i n \sigma^2_{0, i}}b_i^\top \left(\Sigma^{-1} + \sum_{i \in [K]}\frac{\omega_i n}{\sigma^2 + \omega_i n \sigma^2_{0, i}}b_i b_i^\top\right)^{-1}b_k\\
    &= \nu^\top \Sigma^{-1}P^{-1}b_k + \sum_{i \in [K]}\frac{B_i}{\sigma^2 + \omega_i n \sigma^2_{0, i}}b_i^\top P^{-1}b_k\,,
\end{align*}
where we define
\begin{align*}
    P = \Sigma^{-1} + \sum_{i \in [K]}\frac{B_i}{\sigma^2 + \omega_i n \sigma^2_{0, i}}b_i^\top \in\mathbb{R}^{L\times L}\,.
\end{align*}
By linearity,
\begin{align*}
    \E{}{\hat\mu_k} &= \frac{\sigma^2}{\sigma^2_{0, k}\omega_k n +\sigma^2}\left(\nu^\top \Sigma^{-1}P^{-1}b_k + \sum_{i \in [K]}\frac{\E{}{B_i} }{\sigma^2 + \omega_i n \sigma^2_{0, i}}b_i^\top P^{-1}b_k\right) + \frac{\sigma^2_{0, k}}{\sigma^2_{0, k} \omega_k n + \sigma^2}\E{}{B_k}\,.
\end{align*}
From \cref{eq:marginal posterior hierarchical}, $\E{}{B_i} = \omega_i n \nu^\top b_i$:
\begin{align}
    \E{}{\hat\mu_k}  &= \frac{\sigma^2}{\sigma^2_{0, k}\omega_k n +\sigma^2}\left(\nu^\top \Sigma^{-1}P^{-1}b_k + \sum_{i \in [K]}\frac{  \omega_i n \nu^\top b_i}{\sigma^2 + \omega_i n \sigma^2_{0, i}}b_i^\top P^{-1}b_k\right) + \frac{\sigma^2_{0, k}}{\sigma^2_{0, k} \omega_k n + \sigma^2}\omega_k n \nu^\top b_k\nonumber\\
    &= \nu^\top b_k
\end{align}
Now we are ready to compute $\mathbb{V}(\hat\mu_i + \hat\mu_j)$ for any pair of arms $(i, j)$. From \eqref{eq:model_gaussian},
\begin{align*}
    &\hat\mu_i + \hat\mu_j = \frac{\sigma^2}{\sigma^2_{0, i}\omega_i n + \sigma^2}\hat\mu^\top b_i + \frac{\sigma^2_{0, i}}{\sigma^2_{0, i}\omega_i n + \sigma^2}B_i +  \frac{\sigma^2}{\sigma^2_{0, j}\omega_j n + \sigma^2}\hat\mu^\top b_j + \frac{\sigma^2_{0, j}}{\sigma^2_{0, i}\omega_j n + \sigma^2}B_j\\
    &= \frac{\sigma^2}{\sigma^2_{0, i}\omega_i n + \sigma^2}\nu^\top \Sigma^{-1}P^{-1}b_i+ \frac{\sigma^2}{\sigma^2_{0, j}\omega_j n + \sigma^2}\nu^\top \Sigma^{-1}P^{-1}b_j   \\
    &+\underbrace{\frac{\sigma^2}{\sigma^2_{0, i}\omega_i n + \sigma^2}.\sum_{k \in [K]}\frac{B_k}{\omega_k n \sigma^2_{0, k}+\sigma^2}b_k^\top P^{-1}b_i}_{\textcolor{blue}{(a)}} + \underbrace{\frac{\sigma^2}{\sigma^2_{0, j}\omega_j n + \sigma^2}.\sum_{k \in [K]}\frac{B_k}{\omega_k n \sigma^2_{0, k}+\sigma^2}b_k^\top P^{-1}b_j}_{\textcolor{blue}{(b)}} \\
    &+\underbrace{\frac{\sigma^2_{0, j}}{\sigma^2_{0, i}\omega_i n + \sigma^2}B_i}_{\textcolor{blue}{(c)}}+ \underbrace{\frac{\sigma^2_{0, j}}{\sigma^2_{0, j}\omega_j n + \sigma^2}B_j}_{\textcolor{blue}{(d)}}\,.
\end{align*}
But remark that the \textcolor{blue}{(a)}, \textcolor{blue}{(b)},\textcolor{blue}{(c)} and \textcolor{blue}{(d)} are correlated,
\begin{align}
    &\mathbb{V}(\hat\mu_i + \hat\mu_j) = \mathbb{V}\left({\textcolor{blue}{(a)}} + {\textcolor{blue}{(b)}} + {\textcolor{blue}{(c)}} + {\textcolor{blue}{(d)}}\right)\nonumber \\
    &= \sum_{i=1}^4 \mathbb{V}(\textcolor{blue}{(i)}) + \sum_{i=1}^4 \sum_{j=1, j\neq i}^4 2\cov({\textcolor{blue}{(i)}}, {\textcolor{blue}{(j)}})\label{eq:variance_marginal_posterior}\,.
\end{align}

We now compute each term of \eqref{eq:variance_marginal_posterior}:
\begin{align*}
    &\mathbb{V}({\textcolor{blue}{(a)}}) = \frac{\sigma^4}{(\sigma^2_{0, i}\omega_i n + \sigma^2)^2}\mathbb{V}\left( \sum_{k \in [K]}\frac{B_k}{\omega_k n \sigma^2_{0, k}+\sigma^2}b_k^\top P^{-1}b_i \right)\\
    &= \frac{\sigma^4}{(\sigma^2_{0, i}\omega_i n + \sigma^2)^2}\left(\sum_{k \in [K]}\frac{(b_k^\top P^{-1}b_i)^2}{(\sigma^2 + \omega_k n \sigma^2_{0, k})^2}\mathbb{V}(B_k) + \sum_{(k, k^\prime), k\neq k^\prime}\cov\left(\frac{B_k}{\sigma^2 + \omega_k n \sigma^2_{0, k}}b_k^\top P^{-1}b_i, \frac{B_{k^\prime}}{\sigma^2 + \omega_{k^\prime} n \sigma^2_{0, k^\prime}}b_{k^\prime}^\top P^{-1}b_i\right)\right)\\
    &= \frac{\sigma^4}{(\sigma^2_{0, i}\omega_i n + \sigma^2)^2}\left(\sum_{k \in [K]}\frac{((b_k)^\top P^{-1}b_i)^2}{(\sigma^2 + \omega_k n \sigma^2_{0, k})^2}\mathbb{V}(B_k) + \sum_{(k, k^\prime), k\neq k^\prime}\frac{(b_k^\top P^{-1}b_i)(b_{k^\prime}^\top P^{-1}b_i)}{(\sigma^2 + \omega_k n \sigma^2_{0, k})(\sigma^2 + \omega_{k^\prime} n \sigma^2_{0, k^\prime})}\cov(B_k, B_{k^\prime})\right)\,,
    \end{align*}
    \begin{align*}
    \mathbb{V}(\textcolor{blue}{(b)})&= \frac{\sigma^4}{(\sigma^2_{0, j}\omega_j n + \sigma^2)^2}\left(\sum_{k \in [K]}\frac{((b_k)^\top P^{-1}b_j)^2}{(\sigma^2 + \omega_k n \sigma^2_{0, k})^2}\mathbb{V}(B_k) + \sum_{(k, k^\prime), k\neq k^\prime}\frac{(b_k^\top P^{-1}b_i)(b_{k^\prime}^\top P^{-1}b_j)}{(\sigma^2 + \omega_k n \sigma^2_{0, k})(\sigma^2 + \omega_{k^\prime} n \sigma^2_{0, k^\prime})}\cov(B_k, B_{k^\prime})\right)\,,\\
    \mathbb{V}(\textcolor{blue}{(c)})&= \frac{\sigma^4_{0, i}}{(\sigma^2_{0, i}\omega_i n+\sigma^2)^2}\mathbb{V}(B_i)\,,\\
    \mathbb{V}(\textcolor{blue}{(d)})&= \frac{\sigma^4_{0, j}}{(\sigma^2_{0, j}\omega_j n+\sigma^2)^2}\mathbb{V}(B_j)\,,
\end{align*}
\begin{align*}
    \cov( \textcolor{blue}{(a)}, \textcolor{blue}{(b)} ) &= \cov\left( \frac{\sigma^2}{\sigma^2_{0, i}\omega_i n + \sigma^2}.\sum_{k \in [K]}\frac{B_k}{\omega_k n \sigma^2_{0, k}+\sigma^2}b_k^\top P^{-1}b_i, \frac{\sigma^2}{\sigma^2_{0, j}\omega_j n + \sigma^2}.\sum_{k \in [K]}\frac{B_k}{\omega_k n \sigma^2_{0, k}+\sigma^2}b_k^\top P^{-1}b_j \right)\\
    &= \frac{\sigma^4}{(\sigma^2_{0, i}\omega_i n + \sigma^2)(\sigma^2_{0, j}\omega_j n + \sigma^2)}\cov\left( \sum_{k \in [K]}\frac{B_k}{\omega_k n \sigma^2_{0, k}+\sigma^2}b_k^\top P^{-1}b_i, \sum_{k \in [K]}\frac{B_k}{\omega_k n \sigma^2_{0, k}+\sigma^2}b_k^\top P^{-1}b_j  \right)\\
    &=  \frac{\sigma^4}{(\sigma^2_{0, i}\omega_i n + \sigma^2)(\sigma^2_{0, j}\omega_j n + \sigma^2)}\bigg[ \sum_{k \in [K]}\frac{(b_k^\top P^{-1}b_i)(b_k^\top P^{-1}b_j)}{(\sigma^2 + \omega_k n \sigma^2_{0, k})}\mathbb{V}(B_k) \\
    &\qquad\qquad\qquad\qquad\qquad\qquad\qquad\qquad+ \sum_{(k, k^\prime), k\neq k^\prime}\frac{(b_k^\top P^{-1}b_i)(b_{k^\prime}^\top P^{-1}b_j)}{(\sigma^2 + \omega_k n \sigma^2_{0, k})(\sigma^2 + \omega_{k^\prime} n \sigma^2_{0, k^\prime})}\cov(B_k, B_{k^\prime})\bigg]\,,
\end{align*}
\begin{align*}
    \cov( \textcolor{blue}{(c)}, \textcolor{blue}{(d)} ) &= \cov\left(\frac{\sigma^2_{0, i}}{\sigma^2_{0, i}\omega_i n + \sigma^2}B_i, \frac{\sigma^2_{0, j}}{\sigma^2_{0, j}\omega_j n + \sigma^2}B_j \right)\\
    &= \frac{\sigma^2_{0, i}\sigma^2_{0, j}}{(\sigma^2_{0, i}\omega_i n + \sigma^2)(\sigma^2_{0, j}\omega_j n + \sigma^2)}\cov(B_i, B_j)\,,\\
     \cov( \textcolor{blue}{(a)}, \textcolor{blue}{(d)} ) &= \cov\left(\frac{\sigma^2}{\sigma^2_{0, i}\omega_i n + \sigma^2}.\sum_{k \in [K]}\frac{B_k}{\omega_k n \sigma^2_{0, k}+\sigma^2}b_k^\top P^{-1}b_i, \frac{\sigma^2_{0, j}}{\sigma^2_{0, j}\omega_j n + \sigma^2}B_j\right)\\
     &= \frac{\sigma^2 \sigma^2_{0, j}}{(\sigma^2_{0, i}\omega_i n + \sigma^2)(\sigma^2_{0, j}\omega_j n + \sigma^2)}\cov\left( \sum_{k \in [K]}\frac{B_k}{\sigma^2 + \omega_k n \sigma^2_{0, k}}b_k^\top P^{-1}b_i, B_j \right)\\
     &= \frac{\sigma^2 \sigma^2_{0, j}}{(\sigma^2_{0, i}\omega_i n + \sigma^2)(\sigma^2_{0, j}\omega_j n + \sigma^2)}\left[\sum_{k \in [K]\setminus\{j\}} \frac{b_k^\top P^{-1}b_i}{\sigma^2_{0, k}\omega_k n + \sigma^2} + \frac{b_j^\top P^{-1}b_i}{\sigma^2_{0, j}\omega_j n + \sigma^2} \mathbb{V}(B_j) \right]\,.
\end{align*}
The remaining terms are obtained by changing indices of previous terms. Finally, for any arm $(i, j)$ :
\begin{align*}
&\mathbb{V}(B_i) = \mathbb{V}\left(\sum_{t \in \mathcal{A}_i}Y_{t}\right) = \omega_i n \sigma^2 + \omega_i^2 n^2 (\sigma^2_{0, i} + b_i^\top \Sigma b_i)\\
&\cov(B_i, B_j) = \cov\left(\sum_{t\in \mathcal{A}_i}Y_{t}, \sum_{t\in \mathcal{A}_j}Y_{t}\right) = \sum_{t\in \mathcal{A}_i}\sum_{t\in \mathcal{A}_j} \cov(Y_{t}, Y_{t}) = \omega_i \omega_j n^2 b_i^\top \Sigma b_j\,.
\end{align*}
\end{proof}












    \begin{align*}
        &\kappa_j = e^{ -\frac{ \normw{\nu}{(b_m - b_j)(b_m - b_j)^\top}^2 }{c_{j, m}}}\I{j \neq m} + \I{j = m},\,\quad \bSigma_n = \left( \bSigma + \frac{1}{\sigma^2}\sum_{i \in [K]}\omega_i n \bb_i \bb_i^\top \right)^{-1}\\
        & \Bar{\Cova}_n = \frac{1}{\sigma^4}\bSigma_n\left( \sum_{i \in [K]} \omega_i n (\sigma^2 + \bb_i \bSigma \bb_i)\bb_i \bb_i^\top + \doublesum \bb_i \bSigma \bb_j \omega_i \omega_j n^2 \bb_i \bb_j^\top \right)\bSigma_n\,,\quad m=\argmax_{k \in [K]}b_k^\top \nu\,.
    \end{align*}


















\newpage

We begin by stating the complete proof.
%\todon{I do a test whether it's more clear to start from the linear bound and the equivalent model. I report all this proof in a draft. We will ask to Claire and Andras whether it is clearer or not than before. Personally I would prefer to start by the linear bound because it is less computations so maybe more clear.}

\begin{theorem}[Complete statement of \cref{th:upper_bound_hierarchical_model}]
\label{th:complete_upper_bound_hierarchical_model}
    The expected PoE of \emph{\AdaBAIFixed} under the hierarchical Gaussian model in \eqref{eq:model_gaussian} instantiated with arbitrary allocation weights $\omega \in \Delta_K^+$ is upper bounded as
    \begin{align*}
    \mathcal{P}_n \leq \doublesum \frac{\Bar{\kappa}_j}{\sqrt{1 + \frac{ \Bar{c}_{i,j} }{\normw{\bb_i - \bb_j}{\bSigma_n}^2 }}}e^{-\frac{\normw{\nu}{(b_i - b_j)(b_i - b_j)^\top}^2}{2( \normw{b_i - b_j}{\Sigma}^2 + \sigma^2_{0, i}+\sigma^2_{0, j})}}\,,
    \end{align*}
    where
    \begin{align*}
        &\Bar{\kappa}_j = e^{ -\frac{ \normw{\nu}{(b_m - b_j)(b_m - b_j)^\top}^2 }{\Bar{c}_{j, m}}}\I{j \neq m} + \I{j = m},\,\quad \bar{c}_{i, j} = \normw{\bb_i - \bb_j}{\Bar{\Cova}_n}^2,\,\quad \bSigma_n = \left( \bSigma + \frac{1}{\sigma^2}\sum_{i \in [K]}\omega_i n \bb_i \bb_i^\top \right)^{-1}\\
        & \Bar{\Cova}_n = \frac{1}{\sigma^4}\bSigma_n\left( \sum_{i \in [K]} \omega_i n (\sigma^2 + \bb_i \bSigma \bb_i)\bb_i \bb_i^\top + \doublesum \bb_i \bSigma \bb_j \omega_i \omega_j n^2 \bb_i \bb_j^\top \right)\bSigma_n\,,\quad m=\argmax_{k \in [K]}b_k^\top \nu\,.
    \end{align*}
\end{theorem}

\begin{proof}
Recall that we can rewrite a hierarchical bandit \eqref{eq:model_gaussian} as a special instance of a linear bandit \eqref{eq:linear_gaussian},
\begin{talign*}
    \bmu &\sim \cN(\bnu, \bSigma)\nonumber\\
    Y_t \mid \bmu, A_t &\sim \cN(\bb^\top_{A_t} \bmu, \sigma^2)  & \forall t \in [n]\,,
\end{talign*}
where $\Bar{\nu}^T = (\nu, 0, \dots, 0) \in \real^{L+K}$, $\bSigma$ is a block-diagonal matrix  $\bSigma = \langle \Sigma, \sigma^2_{0, 1}, \dots, \sigma^2_{0, K}\rangle \in \real^{L+K, L+K}$  and for any $i \in [K]$, we define the new actions $\bb_i^\top = (b_i^\top, e_i^\top) \in \real^{L+K}$.We remark the following,
\begin{align*}
    \normw{\bb_i - \bb_j}{\bSigma}^2 = \normw{\bb_i - \bb_j}{\Sigma}^2 + \sigma^2_{0, i} + \sigma^2_{0, j},\,\quad \normw{\bnu}{(\bb_i - \bb_j)(\bb_i - \bb_j)^\top}^2 = \normw{\nu}{(b_i - b_j)(b_i - b_j)^\top}^2\,.
\end{align*}

Using \cref{th:linear_model_upper_bound} on this new model and the previous equations gives
\begin{align}
\label{eq:identifying_term_1}
    \mathcal{P}_n &\leq \doublesum \frac{ \left(e^{ -\frac{ \normw{\bnu}{(\bb_m - \bb_j)(\bb_m - \bb_j)^\top}^2 }{\normw{\bb_i - \bb_j}{\Bar{\Cova}_n}^2}}\I{j \neq m} + \I{j = m}\right) e^{- \frac{\normw{\bnu}{(\bb_i - \bb_j)(\bb_i - \bb_j)^\top}^2}{2( \normw{\bb_i - \bb_j}{\bSigma}^2 }}}{\sqrt{1 + \frac{ \normw{\bb_i - \bb_j}{\Bar{\Cova}_n}^2 }{\normw{\bb_i - \bb_j}{\bSigma_n}^2 }}} \nonumber\\
    &= \doublesum \frac{\Bar{\kappa}_j e^{- \frac{\normw{\nu}{(b_i - b_j)(b_i - b_j)^\top}^2}{2( \normw{b_i - b_j}{\Sigma}^2 + \sigma^2_{0, i}+\sigma^2_{0, j})}}}{\sqrt{1 + \frac{ \Bar{c}_{ij} }{\normw{\bb_i - \bb_j}{\bSigma_n}^2 }}}\,.
\end{align}
In order to compute $\Bar{\Sigma}_n$, we remark th

\end{proof}

\newpage

==> introduction.tex <==
\section{INTRODUCTION}\label{sec:introduction}
Best arm identification (BAI) addresses the challenge of finding the optimal arm in a bandit environment \citep{lattimore2020bandit}, with wide-ranging applications in online advertising, drug discovery or hyperparameter tuning. BAI is commonly approached through two primary paradigms: \textit{fixed-confidence} and \textit{fixed-budget}. In the fixed-confidence setting \citep{even2006action,kaufmann2016complexity}, the objective is to find the optimal arm with a pre-specified confidence level. Conversely, fixed-budget BAI \citep{audibert2010best, karnin2013almost, carpentier2016tight} involves identifying the optimal arm within a fixed number of observations. Within this fixed-budget context, two main metrics are used: the probability of error (PoE) \citep{audibert2010best, karnin2013almost, carpentier2016tight}-the likelihood of incorrectly identifying the optimal arm-and the simple regret \citep{bubeck2009pure, russo2016simple, komiyama2023rate}-the expected performance disparity between the chosen and the optimal arm. We study PoE minimization in fixed-budget BAI.

Existing algorithms for PoE minimization in fixed-budget BAI are largely frequentist and often employ elimination strategies. Bayesian approaches have focused on the minimization of the simple regret \citep{komiyama2023rate, azizi2023meta}, or were studied under a frequentist lens \citep{hoffman2014correlation}, which do not capture the advantages of knowing informative priors. It was only recently that \citet{atsidakou2022bayesian} introduced a Bayesian version of the Sequential Halving (SH) algorithm \citep{karnin2013almost}, offering a prior-dependent bound on the probability of error in multi-armed bandits (MAB), albeit under limiting assumptions on the prior. Their proofs are still largely influenced by frequentist approaches and have strong constraints. 

On the other hand, several recent works have shed new light on adaptive methods for frequentist fixed-budget BAI. For instance, \citet{qin2022open,degenne2023existence,wang2023uniformly} examined whether adaptive algorithms can consistently surpass the best non-adaptive algorithm for any bandit instance. \citet{degenne2023existence} established the absence of such universally superior adaptive algorithms in several BAI problems, including Gaussian BAI. \citet{wang2023uniformly} demonstrated that no algorithm consistently outperforms uniform sampling in Bernoulli BAI with two arms. Inspired by these recent results, we develop a method based on fixed and non-adaptive allocations in the Bayesian setting. Instead, our strategy leverages both prior information and the structure of the environment. Our experiments in \cref{sec:experiments} demonstrate that our non-adaptive but prior-informed algorithm can outperform adaptive baselines. Moreover, our proofs incorporate fully Bayesian techniques, diverging from existing works. These techniques apply under milder assumptions, are valid in structured bandit settings, and produce a tighter upper bound that matches known lower bounds up to logarithmic factors.

%As a motivating example, consider a scenario with three arms ($K=3$), where the information \emph{a priori} strongly suggests that either of the first two arms is more likely to be optimal than the third one. Then, how much budget should be allocated to the seemingly suboptimal third arm? Furthermore, if greater confidence is placed on the first arm compared to the second, what is the optimal budget distribution between them? This underlines a fundamental challenge not directly addressed by frequentist approaches, which lack knowledge about the bandit instance before interaction. 

As a motivating example, consider a scenario with three arms (\(K=3\)), where prior information strongly suggests that either of the first two arms is more likely to be optimal than the third. Then, how much budget should be allocated to the seemingly suboptimal third arm? Moreover, if there is greater confidence in the first arm compared to the second, what is the optimal budget distribution between them? This highlights a fundamental challenge not directly addressed by frequentist approaches, which do not incorporate prior knowledge about the bandit instance before interaction.

\textbf{Relation to prior works.} \citet{atsidakou2022bayesian} incorporate prior information, but their method does not fully leverage it as they impose restrictive assumptions on the prior. Also, their algorithm uses a specific budget allocation, whereas ours is general and can be applied with any fixed budget allocation. This flexibility allows for the development of custom allocation strategies, informed by our prior-dependent heuristics or theoretical findings. Moreover, a relevant application of prior information is in structured problems, such as linear bandits \citep{abbasi-yadkori11improved} and hierarchical bandits \citep{hong22hierarchical}, where arm rewards are influenced by underlying \emph{latent} parameters. Our approach incorporates the structure of these problems as reflected in the prior, resulting in more efficient exploration due to arm correlations. This aspect of our work extends beyond the scope of \citet{atsidakou2022bayesian}, which only addressed MAB.

\textbf{Contributions.} \textbf{1)} We present and analyze Prior-Informed BAI, \AdaBAI, a fixed-budget BAI algorithm that leverages prior information for efficient exploration. Our main contributions include establishing prior-dependent upper bounds on its expected PoE in multi-armed, linear, and hierarchical bandits. Specifically, in the MAB setting, our upper bound is tighter and valid under milder assumptions on the prior than \citet{atsidakou2022bayesian}. \textbf{2)} The proof techniques developed for \AdaBAI provide a fully Bayesian perspective, significantly diverging from existing proofs that rely on frequentist techniques. This allows a more comprehensive framework for understanding and analyzing Bayesian BAI algorithms, while also enabling us to relax previously held assumptions. \textbf{3)} Our algorithms and proofs are naturally applicable to structured problems, such as linear and hierarchical bandits, leading to the first Bayesian BAI algorithm with a prior-dependent PoE bound in these settings. \textbf{4)}  We empirically evaluate \AdaBAI's variants in numerous setups. Our experiments on synthetic and real-world data show the generality of \AdaBAI and highlight its good performance.
